Motorway Traffic Flow Prediction using Advanced Deep Learning

Congestion prediction represents a major priority for traffic management centres around the world to ensure timely incident response handling. The increasing amounts of generated traffic data have been used to train machine learning predictors for traffic, however this is a challenging task due to inter-dependencies of traffic flow both in time and space. Recently, deep learning techniques have shown significant prediction improvements over traditional models, however open questions remain around their applicability, accuracy and parameter tuning. This paper proposes an advanced deep learning framework for simultaneously predicting the traffic flow on a large number of monitoring stations along a highly circulated motorway in Sydney, Australia, including exit and entry loop count stations, and over varying training and prediction time horizons. The spatial and temporal features extracted from the 36.34 million data points are used in various deep learning architectures that exploit their spatial structure (convolutional neuronal networks), their temporal dynamics (recurrent neuronal networks), or both through a hybrid spatio-temporal modelling (CNN-LSTM). We show that our deep learning models consistently outperform traditional methods, and we conduct a comparative analysis of the optimal time horizon of historical data required to predict traffic flow at different time points in the future.

==> sections/fig-average-traffic-flow-map.tex <==
%!TEX root = ../IEEE_ITSC_2019.tex
%
\begin{figure}[tbp]
	\centering
	%\framebox{\parbox{3in}{Figures\Fig_1_Rd_network.eps}}
%	\includegraphics[scale=0.22]{Fig_6_Average_congestion_map_from_stations_MS009002A_to_MS009081A_in_Monday}
	\includegraphics[width=.45\textwidth]{Average-traffic-flow-SQUARRE}
    
	\caption{
      	Colormap of average Monday traffic flow on M7.
      	The x-axis is time, and the y-axis represents the 104 A stations (south-bound).
      	The color scale indicates the traffic, between 0 and 1 as it is normalised by the highest traffic.
	}
	\label{fig:average-traffic-flow}
\end{figure}  

==> sections/fig-daily-profile.tex <==
%!TEX root = ../IEEE_ITSC_2019.tex
%
\begin{figure}[tbp]
	\centering
	%\framebox{\parbox{3in}{Figures\Fig_1_Rd_network.eps}}
	\includegraphics[scale=0.45]{Figures/Fig_4a_b_Average_flow.eps}
	\caption{
      	Daily profile for a section.
      	\textbf{(a)} Mean (solid line) and the $20\%-80\%$ percentiles (red area) for the traffic flow series for the station MS009050A, computed on the period 2017-02-01 to 04-30;
      	\textbf{(b)} The daily profiles for station MS009002A for each of the days of the week, computed for the same period of time.
%      	a) Daily average profiling of flow count data 
%      	b) Tuesday average profiling with outlier data. \verify{this might get out as we don't have space; I propose to make an extension of this paper for a journal in which we can discuss all ANOMALIES and prediction performance for outliers}
	}
	\label{fig:daily-profile}
\end{figure}
